Andreev bound states in Superconductor-quantum dot Josephson junction at infinite-U limit

Andreev bound states (ABSs) are studied in quantum dot coupled to conventional BCS superconducting leads on the basis of effective slave boson Hamiltonian in an infinite-U (Coulomb interaction) limit followed by Green's function technique. From the relevant Green's function, density of states (DOS) is analyzed at different superconducting phase differences. On the basis of numerical computation, it is pointed out from DOS plot that ABSs (sub-gap states) arise due to the phase difference between left and right superconducting leads. Due to the dependence on superconducting phase difference, ABSs are current carrying states. We have also analyzed the energy of ABSs as a function of phase difference between left and right superconducting lead for electron hole symmetric as well as non symmetric cases at various dot-lead coupling strengths. It is also pointed out that a finite internal gap arises between upper and lower Andreev bound states in the absence of electron-hole or left-right symmetry. These results are viewed in the light of existing theoretical analysis.

==> references.tex <==
@article{chui,
  title = {Possible realization of entanglement, logical gates, and quantum-information transfer with superconducting-quantum-interference-device qubits in cavity QED},
  author = {Yang, Chui-Ping and Chu, Shih-I and Han, Siyuan},
  journal = {Phys. Rev. A},
  volume = {67},
  issue = {4},
  pages = {042311},
  numpages = {8},
  year = {2003},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.67.042311},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.67.042311}
}



@article{Lh2,
  title = {Carbon Nanotubes as Cooper-Pair Beam Splitters},
  author = {Herrmann, L. G. and Portier, F. and Roche, P. and Yeyati, A. Levy and Kontos, T. and Strunk, C.},
  journal = {Phys. Rev. Lett.},
  volume = {104},
  issue = {2},
  pages = {026801},
  numpages = {4},
  year = {2010},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.104.026801},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.104.026801}
}

 . Nature 453, 1031–1042 (2008).

@article{john,
  title={Superconducting quantum bits},
  author={Clarke, J., Wilhelm, F.},
  journal={Nature},
  volume={453},
  number={1},
  pages={1031},
  year={2008},
  publisher={APS}
}


@article{Josephson,
  title={Coupled superconductors},
  author={Josephson, BD},
  journal={Reviews of Modern Physics},
  volume={36},
  number={1},
  pages={216},
  year={1964},
  publisher={APS}
}

@article{Reed,
  title={Quantum dots},
  author={Reed, Mark A},
  journal={Scientific American},
  volume={268},
  number={1},
  pages={118--123},
  year={1993},
  publisher={JSTOR}
}


@article{Yashai,
  title={Tunneling through an Anderson impurity between superconductors},
  author={Avishai, Yshai and Golub, Anatoly and Zaikin, Andrei D},
  journal={Physical Review B},
  volume={63},
  number={13},
  pages={134515},
  year={2001},
  publisher={APS}
}

@article{yuzhu,
  title={Andreev bound states and the $\pi$-junction transition in a superconductor/quantum-dot/superconductor system},
  author={Zhu, Yu and Sun, Qing-feng and Lin, Tsung-han},
  journal={Journal of Physics: Condensed Matter},
  volume={13},
  number={39},
  pages={8783},
  year={2001},
  publisher={IOP Publishing}
}

@article{AKumar,
  title={Temperature dependence of Andreev spectra in a superconducting carbon nanotube quantum dot},
  author={Kumar, A and Gaim, M and Steininger, D and Yeyati, A Levy and Mart{\'\i}n-Rodero, A and H{\"u}ttel, AK and Strunk, Ch},
  journal={Physical Review B},
  volume={89},
  number={7},
  pages={075428},
  year={2014},
  publisher={APS}
}

@article{JDPillet,
  title={Andreev bound states in supercurrent-carrying carbon nanotubes revealed},
  author={Pillet, JD and Quay, CHL and Morfin, P and Bena, C and Yeyati, A Levy and Joyez, P},
  journal={Nature Physics},
  volume={6},
  number={12},
  pages={965--969},
  year={2010},
  publisher={Nature Publishing Group}
}

@article{Kondo,
  title={Resistance minimum in dilute magnetic alloys},
  author={Kondo, Jun},
  journal={Progress of theoretical physics},
  volume={32},
  number={1},
  pages={37--49},
  year={1964},
  publisher={Oxford University Press}
}

@article{Bumkim,
  title={Transport measurement of andreev bound states in a kondo-correlated quantum dot},
  author={Kim, Bum-Kyu and Ahn, Ye-Hwan and Kim, Ju-Jin and Choi, Mahn-Soo and Bae, Myung-Ho and Kang, Kicheon and Lim, Jong Soo and L{\'o}pez, Rosa and Kim, Nam},
  journal={Physical review letters},
  volume={110},
  number={7},
  pages={076803},
  year={2013},
  publisher={APS}
}

@article{Joshua,
  title={Proximity-induced Shiba states in a molecular junction},
  author={Island, Joshua O and Gaudenzi, Rocco and De Bruijckere, Joeri and Burzur{\'\i}, Enrique and Franco, Carlos and Mas-Torrent, Marta and Rovira, Concepci{\'o} and Veciana, Jaume and Klapwijk, Teun M and Aguado, Ram{\'o}n and others},
  journal={Physical Review Letters},
  volume={118},
  number={11},
  pages={117001},
  year={2017},
  publisher={APS}
}

@article{KJ,
  title={Competition of superconducting phenomena and Kondo screening at the nanoscale},
  author={Franke, KJ and Schulze, G and Pascual, JI},
  journal={Science},
  volume={332},
  number={6032},
  pages={940--944},
  year={2011},
  publisher={American Association for the Advancement of Science}
}

@article{Rok,
  title = {Josephson Current in Strongly Correlated Double Quantum Dots},
  author = {\ifmmode \check{Z}\else \v{Z}\fi{}itko, Rok and Lee, Minchul and L\'opez, Rosa and Aguado, Ram\'on and Choi, Mahn-Soo},
  journal = {Phys. Rev. Lett.},
  volume = {105},
  issue = {11},
  pages = {116803},
  numpages = {4},
  year = {2010},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.105.116803},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.105.116803}
}





@article{Jorden,
  title={Supercurrent reversal in quantum dots},
  author={Van Dam, Jorden A and Nazarov, Yuli V and Bakkers, Erik PAM and De Franceschi, Silvano and Kouwenhoven, Leo P},
  journal={Nature},
  volume={442},
  number={7103},
  pages={667--670},
  year={2006},
  publisher={Nature Publishing Group}
}

@article{silvano,
  title={Hybrid superconductor--quantum dot devices},
  author={De Franceschi, Silvano and Kouwenhoven, Leo and Sch{\"o}nenberger, Christian and Wernsdorfer, Wolfgang},
  journal={Nature Nanotechnology},
  volume={5},
  number={10},
  pages={703},
  year={2010},
  publisher={Nature Publishing Group}
}


@article{H,
  title={Critical current 0- $\pi$ transition in designed Josephson quantum dot junctions},
  author={J{\o}rgensen, H Ingerslev and Novotn{\`y}, T and Grove-Rasmussen, Kasper and Flensberg, Karsten and Lindelof, Poul Erik},
  journal={Nano letters},
  volume={7},
  number={8},
  pages={2441--2445},
  year={2007},
  publisher={ACS Publications}
}


@article{AYu,
  title={Proximity effect in a superconductor-metallofullerene-superconductor molecular junction},
  author={Kasumov, A Yu and Tsukagoshi, K and Kawamura, M and Kobayashi, T and Aoyagi, Y and Senba, K and Kodama, T and Nishikawa, H and Ikemoto, I and Kikuchi, K and others},
  journal={Physical Review B},
  volume={72},
  number={3},
  pages={033414},
  year={2005},
  publisher={APS}
}


@article{HI,
  title={Critical current 0- $\pi$ transition in designed Josephson quantum dot junctions},
  author={J{\o}rgensen, H Ingerslev and Novotn{\`y}, T and Grove-Rasmussen, Kasper and Flensberg, Karsten and Lindelof, Poul Erik},
  journal={Nano letters},
  volume={7},
  number={8},
  pages={2441--2445},
  year={2007},
  publisher={ACS Publications}
}

@article{Pillet,
  title={Tunneling spectroscopy of a single quantum dot coupled to a superconductor: From Kondo ridge to Andreev bound states},
  author={Pillet, J-D and Joyez, P and Goffman, MF and others},
  journal={Physical Review B},
  volume={88},
  number={4},
  pages={045101},
  year={2013},
  publisher={APS}
}



@article{Minchu,
  title={Kondo effect and Josephson current through a quantum dot between two superconductors},
  author={Choi, Mahn-Soo and Lee, Minchul and Kang, Kicheon and Belzig, Wolfgang},
  journal={Physical Review B},
  volume={70},
  number={2},
  pages={020502},
  year={2004},
  publisher={APS}
}

@article{Tanaka,
  title={Kondo effect in asymmetric Josephson couplings through a quantum dot},
  author={Tanaka, Yoshihide and Oguri, Akira and Hewson, AC},
  journal={New Journal of Physics},
  volume={9},
  number={5},
  pages={115},
  year={2007},
  publisher={IOP Publishing}
}

@article{DJ,
  title={Understanding the Josephson current through a Kondo-correlated quantum dot},
  author={Luitz, David J and Assaad, Fakher F and Novotn{\`y}, Tom{\'a}{\v{s}} and Karrasch, Christoph and Meden, Volker},
  journal={Physical review letters},
  volume={108},
  number={22},
  pages={227001},
  year={2012},
  publisher={APS}
}

@article{RD,
  title={Manipulating the magnetic state of a carbon nanotube Josephson junction using the superconducting phase},
  author={Delagrange, R and Luitz, DJ and Weil, R and Kasumov, A and Meden, V and Bouchiat, H and Deblock, R},
  journal={Physical Review B},
  volume={91},
  number={24},
  pages={241401},
  year={2015},
  publisher={APS}
}

@article{Aashish,
  title={Loss of $\pi$-junction behavior in an interacting impurity Josephson junction},
  author={Clerk, Aashish A and Ambegaokar, Vinay},
  journal={Physical Review B},
  volume={61},
  number={13},
  pages={9109},
  year={2000},
  publisher={APS}
}

@article{Martin,
  title={Josephson and Andreev transport through quantum dots},
  author={Mart{\'\i}n-Rodero, A and Levy Yeyati, A},
  journal={Advances in Physics},
  volume={60},
  number={6},
  pages={899--958},
  year={2011},
  publisher={Taylor \& Francis}
}

@article{satoshi,
  title={dc Josephson current through a quantum dot coupled with superconducting leads},
  author={Ishizaka, Satoshi and Sone, Jun’ichi and Ando, Tsuneya},
  journal={Physical Review B},
  volume={52},
  number={11},
  pages={8358},
  year={1995},
  publisher={APS}
}

@article{EVecino,
  title={Josephson current through a correlated quantum level: Andreev states and $\pi$ junction behavior},
  author={Vecino, E and Mart{\'\i}n-Rodero, A and Yeyati, A Levy},
  journal={Physical Review B},
  volume={68},
  number={3},
  pages={035105},
  year={2003},
  publisher={APS}
}

@article{JF,
  title={Nonequilibrium transport through a Josephson quantum dot},
  author={Rentrop, Jan F and Jakobs, Severin G and Meden, Volker},
  journal={Physical Review B},
  volume={89},
  number={23},
  pages={235110},
  year={2014},
  publisher={APS}
}

@article{Gagan,
  title={Tunable Josephson effect in hybrid parallel coupled double quantum dot-superconductor tunnel junction},
  author={Rajput, Gagan and Kumar, Rajendra and others},
  journal={Superlattices and Microstructures},
  volume={73},
  pages={193--202},
  year={2014},
  publisher={Elsevier}
}

@article{YAvishai,
  title={Superconductor-quantum dot-superconductor junction in the Kondo regime},
  author={Avishai, Yshai and Golub, Anatoly and Zaikin, Andrei D},
  journal={Physical Review B},
  volume={67},
  number={4},
  pages={041301},
  year={2003},
  publisher={APS}
}

@article{ALYeyati,
  title={Nonequilibrium dynamics of andreev states in the kondo regime},
  author={Yeyati, A Levy and Mart{\'\i}n-Rodero, A and Vecino, E},
  journal={Physical review letters},
  volume={91},
  number={26},
  pages={266802},
  year={2003},
  publisher={APS}
}

@book{Hewson,
  title={The Kondo problem to heavy fermions},
  author={Hewson, Alexander Cyril},
  volume={2},
  year={1997},
  publisher={Cambridge university press}
}


